HEART: Exploiting Head Heterogeneity in Sparse Attention for Video Diffusion

Sparse attention accelerates video diffusion by allowing each attention head to focus on only a small subset of interactions. Existing methods already construct head-specific sparse patterns conditioned on the input. However, we find that these heads also differ in two less obvious but practically important ways. First, for some heads, sparse attention masks remain stable across many denoising steps, whereas others change rapidly. Second, heads differ substantially in their sensitivity to sparsification: applying the same threshold can induce markedly different errors in the final denoising velocity. Ignoring these differences leads to redundant mask prediction and suboptimal threshold calibration across heads under a global sparsity budget. We present HEART, short for Heterogeneity-Exploiting Adaptive Refresh and Thresholding, a training-free framework that exploits both forms of head heterogeneity. First, Temporal Mask Reuse (TMR) uses a lightweight per-head query-key drift signal to determine whether a cached sparse mask remains reliable across denoising steps, refreshing it only when the drift exceeds a prescribed threshold. Second, Error-guided Budgeted Calibration (EBC) evaluates candidate thresholds offline using a frequency-weighted denoising-velocity error, and assigns each head an appropriate threshold under a global sparsity budget. HEART requires no retraining, weight modification, or sparse-kernel changes, and can be integrated directly into existing sparse-attention pipelines. Across Wan2.1-1.3B, Wan2.1-14B, and HunyuanVideo-13B, HEART consistently pushes the quality--efficiency frontier of advanced sparse attention methods such as XAttention and SVG2 outward.

==> template/mac_automl_core.tex <==
% =============================================================================
% MAC-AutoML core template
% Public responsibility:
% 1. Load all shared packages and layout rules.
% 2. Expose shared front-matter and header/footer configuration APIs.
% 3. Keep all theme-independent visual logic in one place.
%
% Theme wrappers are expected to define:
% - \macframecolordef
% - \macaccentcolordef
% - \macaccenttext
% =============================================================================

\@ifundefined{macframecolordef}{\ClassError{\@classname}{Missing theme hook \string\macframecolordef}{Define it in the theme .cls before loading mac_automl_core.tex}}{}
\@ifundefined{macaccentcolordef}{\ClassError{\@classname}{Missing theme hook \string\macaccentcolordef}{Define it in the theme .cls before loading mac_automl_core.tex}}{}
\@ifundefined{macaccenttext}{\ClassError{\@classname}{Missing theme hook \string\macaccenttext}{Define it in the theme .cls before loading mac_automl_core.tex}}{}

\LoadClassWithOptions{article}
\RequirePackage{iftex}
\ifdefined\pdfoutput
\pdfoutput=1
\fi

% =============================================================================
% Core packages and layout
% =============================================================================

\RequirePackage[top=2.12cm, bottom=3.20cm, left=2.5cm, right=2.5cm, columnsep=0.65cm]{geometry}
\ifXeTeX\else
\RequirePackage{microtype}
\fi
\RequirePackage{placeins}
\RequirePackage{setspace}
\RequirePackage{parskip}
\RequirePackage[english]{babel}
\RequirePackage{lipsum}
\RequirePackage{etoolbox}
\RequirePackage{enumitem}
\newcommand{\nohyphens}{\hyphenpenalty=10000\exhyphenpenalty=10000\relax}

\RequirePackage{fancyhdr}
\ifdefined\pdfoutput
\DisableLigatures[f]{family=sf*}
\fi

% =============================================================================
% Graphics
% =============================================================================

\RequirePackage{graphicx}
\RequirePackage[export]{adjustbox}
\RequirePackage{subcaption}

% =============================================================================
% Tables
% =============================================================================

\RequirePackage{booktabs}
\RequirePackage{nicematrix}
\RequirePackage{multirow}
\RequirePackage{makecell}
\RequirePackage{colortbl}
\RequirePackage{bm}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\RequirePackage{pifont}
\RequirePackage{marvosym}
\newcommand{\nm}[1]{#1}

% =============================================================================
% Theme colors
% =============================================================================

\RequirePackage[most]{tcolorbox}
\RequirePackage{xcolor}
\macframecolordef
\macaccentcolordef
\newcommand{\omniaccent}[1]{\macaccenttext{#1}}
\definecolor{black}{rgb}{0,0,0}
\newcommand{\black}[1]{{\bfseries\color[HTML]{000000} #1}}

% =============================================================================
% References
% =============================================================================

\RequirePackage{hyperref}
\RequirePackage{xurl}
\RequirePackage[noabbrev,nameinlink]{cleveref}
\hypersetup{
  colorlinks,
  linkcolor=omniaccent,
  citecolor=omniaccent,
  urlcolor=omniaccent
}

\RequirePackage[numbers, sort&compress]{natbib}
\def\bibfont{\small}
\special{pdf:minorversion 7}
\emergencystretch=1.5em
\hbadness=2000

% =============================================================================
% Bibliography
% =============================================================================
\addto{\captionsenglish}{\renewcommand{\refname}{References}}
\newcommand{\citeas}[1]{\Needspace*{8\baselineskip}\noindent\bibentry{#1}}

% =============================================================================
% Section and caption style
% =============================================================================

\newcommand{\sectionfont}
{\fontsize{13}{14}\selectfont}

\newcommand{\subsectionfont}
{\fontsize{11}{13}\selectfont}

\RequirePackage{titlesec}
\titleformat*{\paragraph}{\itshape}
\titleformat*{\section}{\sectionfont\sffamily\bfseries\omniaccent}
\titleformat*{\subsection}{\subsectionfont\sffamily\bfseries\omniaccent}
\titleformat*{\subsubsection}{\normalsize\sffamily\bfseries\omniaccent}
\titlespacing*{\section}{0pt}{3ex plus4pt minus3pt}{5pt}
\titlespacing*{\subsection}{0pt}{2.5ex plus3pt minus2pt}{2pt}
\titlespacing*{\subsubsection}{0pt}{2ex plus2.5pt minus1.5pt}{2pt}

\RequirePackage{caption}
\DeclareCaptionLabelSeparator{period}{. }
\captionsetup{
  labelfont={bf,sf},
  labelsep=period,
  figurename=Figure,
  tablename=Table,
  format=plain,
  singlelinecheck=off,
  justification=raggedright,
  font=small
}
\captionsetup[figure]{
  skip=6pt,
  format=plain,
  singlelinecheck=off,
  justification=raggedright
}
\captionsetup[table]{
  skip=4pt,
  format=plain,
  singlelinecheck=off,
  justification=raggedright
}

\ifXeTeX
  \RequirePackage{fontspec}
  \setmainfont[
    SmallCapsFeatures = {Letters=SmallCaps}
  ]{TeX Gyre Termes}
  \setsansfont{Noto Sans}
  \setmonofont{Noto Sans Mono}
  \newfontfamily\omnibytesansmedium[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Medium,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Medium}
  \newfontfamily\omnititlefont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniheadingfont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniauthorfont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniaffiliationfont{Noto Sans}
  \newfontfamily\omniemailfont{Noto Sans}
  \newfontfamily\omnimonofont{Noto Sans Mono}
\else
  \RequirePackage[T1]{fontenc}
  \renewcommand{\sfdefault}{lmss}%
  \renewcommand{\rmdefault}{cmr}
\fi

% =============================================================================
% Front-matter data model
% =============================================================================

\renewcommand\addtolist[5][]{
  \begingroup
    \if\relax#3\relax\def\sep{}\else\def\sep{#5}\fi
    \let\protect\@unexpandable@protect
    \xdef#3{\expandafter{#3}\sep #4[#1]{#2}}%
  \endgroup
}

\newcommand{\authorfont}
{\fontsize{12}{14}\selectfont}

\newcommand{\authorgroupfont}
{\fontsize{9.1}{10.8}\selectfont}
\newcommand{\affmark}[1]{\textsuperscript{#1}}

\newcommand\authorlist{}
\ifXeTeX
\newcommand\authorformat[2][]{\authorfont {\color{black!84}\omniauthorfont\bfseries #2\affmark{#1}}}
\else
\newcommand\authorformat[2][]{\authorfont {\color{black!82}\sffamily\mdseries #2\affmark{#1}}}
\fi
\renewcommand\author[2][]{\addtolist[#1]{#2}{\authorlist}{\authorformat}{, }}

\newcommand{\affiliationfont}
{\fontsize{10}{12}\selectfont}

\newcommand\affiliationlist{}
\ifXeTeX
\newcommand\affiliationformat[2][]{{\affiliationfont {\omniaffiliationfont \affmark{#1}#2}}}
\else
\newcommand\affiliationformat[2][]{{\affiliationfont {\sffamily \affmark{#1}#2}}}
\fi
\newcommand\affiliation[2][]{\addtolist[#1]{#2}{\affiliationlist}{\affiliationformat}{, }}

\newcommand{\contributionfont}
{\fontsize{9.6}{12}\selectfont}

\newcommand\contributionlist{}
\newcommand\contributionformat[2][]{{\contributionfont \affmark{#1}#2}}
\newcommand\contribution[2][]{\addtolist[#1]{#2}{\contributionlist}{\contributionformat}{, }}

\newcommand{\emailfont}
{\fontsize{8.2}{10.4}\selectfont}

\newcommand\emaillist{}
\ifXeTeX
\newcommand\emails[1]{\def\emaillist{{\emailfont\color{black!60}\omniemailfont #1}}}
\else
\newcommand\emails[1]{\def\emaillist{{\emailfont\color{black!65}\ttfamily #1}}}
\fi

\newcommand{\checkdatafont}
{\fontsize{7.92}{10}\selectfont}

\newcommand\checkdatalist{}
\newcommand\checkdataformat[2][]{{\small {\checkdatafont\sffamily \bfseries #1:} #2}}
\newcommand\checkdata[2][]{\addtolist[#1]{#2}{\checkdatalist}{\checkdataformat}{\par}}

\newcommand{\abstractinfont}
{\fontsize{10}{12}\selectfont}

\renewcommand{\abstract}[1]{\def\abstractlist{{\abstractinfont #1}}}
\newcommand{\email}[1]{\href{mailto:#1}{\texttt{#1}}}
\newcommand{\corremailmark}{\Letter}
\newcommand{\authormark}[1]{\textsuperscript{#1}}
\newcommand{\authorentry}[2]{\mbox{#1\authormark{#2}}}
\newcommand{\authorsep}{\hspace{0.78em}}
\newcommand{\authorrow}[1]{\makebox[\linewidth][c]{#1}\par\vspace{2.2pt}}
\newcommand{\affiliationline}[1]{#1\par}
\newcommand{\contactline}[1]{#1\par}

\newcommand{\macauthorrows}{}
\newcommand{\macaffiliationrows}{}
\newcommand{\maccontactrows}{}

% Public front-matter configuration API.
\newcommand{\setauthorrows}[1]{\gdef\macauthorrows{#1}}
\newcommand{\setaffiliationrows}[1]{\gdef\macaffiliationrows{#1}}
\newcommand{\setcontactrows}[1]{\gdef\maccontactrows{#1}}
\newcommand{\usecustomauthorlayout}{
  \def\authorlist{%
    {\fontsize{12}{14}\selectfont\color{black!96}%
    \ifXeTeX\omniauthorfont\bfseries\else\sffamily\bfseries\fi
    \parbox{0.96\linewidth}{\centering \macauthorrows}}}
  \def\affiliationlist{%
    {\fontsize{9.9}{11.9}\selectfont\color{black!70}%
    \ifXeTeX\omnibytesansmedium\else\sffamily\fi
    \parbox{0.92\linewidth}{\centering
    \macaffiliationrows\par
    \vspace{2.8mm}
    {\fontsize{9.8}{11.8}\selectfont\color{black!82}%
    \ifXeTeX\omnibytesansmedium\else\sffamily\fi
    \maccontactrows}}}}
  \def\emaillist{{}}}
\newcommand{\setfrontauthors}[1]{\setauthorrows{#1}}
\newcommand{\setfrontaffiliations}[1]{\setaffiliationrows{#1}}
\newcommand{\setfrontcontact}[1]{\setcontactrows{#1}}

\renewcommand\date[1]{\checkdata[Date]{#1}}
\newcommand\correspondence[1]{\checkdata[Correspondence]{#1}}

\newcommand{\titlefont}
{\fontsize{17}{20}\selectfont}

\ifXeTeX
\renewcommand{\title}[1]{\newcommand{\titlelist}{\parbox{0.945\linewidth}{\centering\titlefont{\omnititlefont\bfseries #1}}}}
\else
\renewcommand{\title}[1]{\newcommand{\titlelist}{\parbox{0.92\linewidth}{\centering\titlefont{\sffamily\bfseries #1}}}}
\fi

\newcommand{\abstractfont}
{\fontsize{12}{12}\selectfont}

\ifXeTeX
\newcommand{\beginabstract}{\abstractfont{\omniauthorfont\bfseries\color{omniaccent!88!black}Abstract}}
\else
\newcommand{\beginabstract}{\abstractfont{\sffamily\bfseries\color{omniaccent}\MakeUppercase{Abstract}}}
\fi

\newcommand{\beginappendix}{\appendix{\titlefont\sffamily \omniaccent{Appendix}\par}}
\colorlet{abstractboxfill}{white}

% =============================================================================
% Reusable document-level utilities
% =============================================================================

\newcommand{\macparagraph}[1]{\par\vspace{2pt}\noindent\textbf{#1}\hspace{1.8ex}}
\definecolor{macgreen}{RGB}{34,139,34}
\definecolor{macred}{RGB}{220,20,60}
\definecolor{macorange}{RGB}{255,140,0}
\newcommand{\cmark}{\textcolor{macgreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{macred}{\ding{55}}}
\newcommand{\pmark}{\textcolor{macorange}{\raisebox{0.12ex}{\footnotesize\textasciitilde}}}
\newcommand{\fb}{\makebox[0.5em][c]{\textbullet}}
\newcommand{\eb}{\makebox[0.5em][c]{\textopenbullet}}
\newcommand{\eg}{e.g.,\ }
\newcommand{\ie}{i.e.,\ }

\tcbuselibrary{skins}
\tcbset{
  aibox/.style={
    width=\linewidth,
    top=7pt,
    bottom=2pt,
    colback=blue!4!white,
    colframe=black,
    colbacktitle=black,
    enhanced,
    center,
    attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    boxed title style={boxrule=0pt,colframe=white,},
  }
}
\newtcolorbox{AIbox}[2][]{aibox,title=#2,#1}

% =============================================================================
% Template-level branding configuration
% =============================================================================

\newcommand{\macleftheadercontent}{}
\newcommand{\macrightheadericon}{}
\newcommand{\macrunningheadericon}{}
\newcommand{\macheadertextcontent}{MAC-AutoML}

\newcommand{\setleftheadercontent}[1]{\gdef\macleftheadercontent{#1}}
\newcommand{\setrightheadericon}[1]{\gdef\macrightheadericon{#1}}
\newcommand{\setrunningheadericon}[1]{\gdef\macrunningheadericon{#1}}
\newcommand{\setheadergroupname}[1]{\gdef\macheadertextcontent{#1}}
\newcommand{\headerlogo}[3][0pt]{\raisebox{#1}{\includegraphics[height=#2]{#3}}}
\newcommand{\headerlogospace}[1]{\hspace*{#1}}

% Public header/footer configuration API.
\newcommand{\firstpageheaderlogos}{%
  \makebox[\textwidth][s]{%
    \macleftheadercontent\hfill\macrightheadericon
  }%
}
\ifXeTeX
\newcommand{\omniheadertext}{{\omniauthorfont\fontsize{8.1}{10}\selectfont\color{black!58}\addfontfeatures{LetterSpace=4}\macheadertextcontent}}
\else
\newcommand{\omniheadertext}{\sffamily\fontsize{8.1}{10}\selectfont\color{black!60} \macheadertextcontent}
\fi
\fancypagestyle{firststyle}{
    \fancyhead[L]{
        \vskip 0.8mm
        \firstpageheaderlogos
    }
    \fancyhead[R]{}
}
\pagestyle{fancy}
\fancyhf{}
\fancyhead[L]{
  \vskip 2.5mm
  \macrunningheadericon
}
\fancyhead[R]{
  \vskip 4.2mm
  \omniheadertext
}
\fancyfoot[C]{\sffamily\fontsize{8.6}{10}\selectfont\thepage}

\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}
\setlength{\headheight}{64pt}
\setlength{\headsep}{6pt}
\setlength{\footskip}{18pt}

% =============================================================================
% Title and abstract box implementation
% =============================================================================
\newcommand{\@toptitlebar}{
  {\color{omniaccent!88!black}\hrule height 2.4pt}
  \vskip 6mm
}
\newcommand{\@bottomtitlebar}{
  \vskip 6mm
  {\color{omniaccent!88!black}\hrule height 2.4pt}
}

% Titlebox %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mymaketitle}{%
  \tcbset{enhanced}
  \tcbset{left=8mm}
  \tcbset{right=8mm}
  \tcbset{top=4.0mm}
  \tcbset{bottom=3.8mm}
  \tcbset{colback=white}
  \tcbset{colframe=omniframe}
  \tcbset{boxrule=3pt}
  \tcbset{before skip=0pt}
  \tcbset{grow to left by=1.5pt}
  \tcbset{grow to right by=1.5pt}
  \tcbset{arc=2.2mm}
      {
      \setlength{\parskip}{0mm}
      \hfuzz=20pt
      \hbadness=10000
      \centering
      \nohyphens

      {
      \vspace*{-4.8mm}
      \@toptitlebar

        \titlelist\par
         \@bottomtitlebar
      }
      \vskip 4.0mm
      \authorlist
      \vskip 2.4mm

      \affiliationlist\par
      \ifdefempty{\emaillist}{}{\vskip 3mm \emaillist\par}

      \contributionlist\par
    }
   \vskip 2.6mm

  \begin{tcolorbox}[
    enhanced jigsaw,
    colback=abstractboxfill,
    colframe=omniaccent!99,
    boxrule=1.6pt,
    arc=2.5mm,
    left=8mm,
    right=8mm,
    top=4.1mm,
    bottom=4.2mm,
    interior style={fill=abstractboxfill},
    drop shadow={black!12!white},
    before skip=0pt,
    after skip=0pt
  ]
    \setlength{\parindent}{0cm}
    \setlength{\parskip}{0cm}

    \begin{center}
      \beginabstract
      \vskip 1.8mm
    \end{center}

    \abstractlist\par
    \vskip 0.6mm
    {
      \setlength{\parskip}{0cm}
      \ifdefempty{\checkdatalist}{\vspace*{0.02cm}}{\checkdatalist\par}
    }
  \end{tcolorbox}
  \tcbset{reset}
  \FloatBarrier

  \thispagestyle{firststyle}
}

\if@twocolumn%
\renewcommand{\maketitle}{
\twocolumn[%
 \vskip 2mm
  \mymaketitle
  \vskip 4mm
]
}%
\else%
\renewcommand{\maketitle}{
  \mymaketitle
  \vskip 4mm
}%
\fi

